Going Deeper through the Gleason Scoring Scale: An Automatic end-to-end System for Histology Prostate Grading and Cribriform Pattern Detection

The Gleason scoring system is the primary diagnostic and prognostic tool for prostate cancer. In recent years, with the development of digitisation devices, the use of computer vision techniques for the analysis of biopsies has increased. However, to the best of the authors' knowledge, the development of algorithms to automatically detect individual cribriform patterns belonging to Gleason grade 4 has not yet been studied in the literature. The objective of the work presented in this paper is to develop a deep-learning-based system able to support pathologists in the daily analysis of prostate biopsies. The methodological core of this work is a patch-wise predictive model based on convolutional neural networks able to determine the presence of cancerous patterns. In particular, we train from scratch a simple self-design architecture. The cribriform pattern is detected by retraining the set of filters of the last convolutional layer in the network. From the reconstructed prediction map, we compute the percentage of each Gleason grade in the tissue to feed a multi-layer perceptron which provides a biopsy-level score.mIn our SICAPv2 database, composed of 182 annotated whole slide images, we obtained a Cohen's quadratic kappa of 0.77 in the test set for the patch-level Gleason grading with the proposed architecture trained from scratch. Our results outperform previous ones reported in the literature. Furthermore, this model reaches the level of fine-tuned state-of-the-art architectures in a patient-based four groups cross validation. In the cribriform pattern detection task, we obtained an area under ROC curve of 0.82. Regarding the biopsy Gleason scoring, we achieved a quadratic Cohen's Kappa of 0.81 in the test subset. Shallow CNN architectures trained from scratch outperform current state-of-the-art methods for Gleason grades classification.

==> 03_03_Model_Interpretation.tex <==
\subsection{Model Interpretation}
\label{sectionModelInterp}

One of the main drawbacks about the use of deep learning models in medical practice is the lack of interpretability. This fact creates distrust in the clinicians, the final users of CAD systems. To deal with this gap, in this research we study the interpretability of the trained models by means of Activation Maximisation and Class Activation Maps techniques.


The Activation Maximisation (AM) strategy is introduced in \cite{Erhan2009VisualizatingNetwork} and aims to represent the pattern in the input image that maximises the response of each convolutional filter. This technique is based on the end-to-end differentiability of convolutional neural networks. Once the weights of the CNN-based model have been learned, the activation map $y^j_i[m',n']$ of the filter $i$ in the layer $j$ can be expressed as a function of the input image $x[m,n]$ as follows:

\begin{equation}
\label{eq:MA1}
y_{i}^{j}[m',n'] = h_{i}^{j}(x[m,n])
\end{equation}

The problem of calculating the input image $x^{*}[m,n]$ that obtains the maximum activation $y_{i}^{j}[m',n']$ can be solved as an optimisation problem of certain loss function $L$:

\begin{equation}
\label{eq:MA2}
%x^{*} \quad | \quad \min_{L} \quad L = f(y_{i}^{j}[m',n'])
x^{*} = \arg\min_{m,n} L
\end{equation}

To address this calculation by minimisation of a convex function looking for a local minimum, the loss function defined is: 

\begin{equation}
\label{eq:MA3}
L = -\sum_{m'}\sum_{n'}y_{i}^{j}[m',n']
\end{equation}

The input image $x[m,n]$ is randomly initialised to a Gaussian distribution in the range of $[0, 1]$. The AM image for certain filter is obtained updating the values in the pixels of the initial $x[m,n]$ via Stochastic Gradient Descent up to convergence of the loss function as follows:

\begin{equation}
\label{eq:MA4}
x_{it}[m,n] = x_{it-1}[m,n] - \frac{\partial L}{\partial x_{it-1}[m,n]}
\end{equation}

Regarding the Class Activation Maps (CAM), this strategy was proposed in \cite{Zhou2016LearningLocalization} as a procedure to obtain a heatmap indicating the regions of the input image in which the model is paying attention to predict certain class. This is a useful technique, that allows checking if the network is basing its decision in discriminating patterns. CAM is defined for a concrete image $x[m,n]$, and the class predicted $c$ in architectures in which global-average pooling or global-max pooling is used after the last convolutional layer. Let be $y_{i}[m',n']$ the activation maps output of the last convolutional layer for the input image $x$ classified as $c$, the CAM heatmap could be defined as:

\begin{equation}
\label{eq:CAM1}
CAM^{y} [m',n'] = \sum_{i} w_{i}^{y} * y_{i}[m',n']
\end{equation}

\noindent where $w_{i}^{y}$ weights the contribution of each activation map to the prediction, and they are obtained by the gradient:

\begin{equation}
\label{eq:CAM2}
w_{i}^{y} = \frac{\partial c}{\partial p(y_{i}[m',n'])}
\end{equation}

\noindent being $p(\cdot)$ is the pooling operation used, global-max pooling or global-average pooling to the activation map in the architecture.

In order to obtain a clearer localisation of the relevant activated areas, the heatmap is post-processed. Values below 0 are clipped, the activation values are normalised by its maximum, and a binary mask is obtained with the pixels with at least a $75\%$ of intensity. Finally, the CAM is resized to match the original image dimensions.
